When Less Is More: Consequence-Finding in a Weak Theory of Arithmetic

This paper presents a theory of non-linear integer/real arithmetic and algorithms for reasoning about this theory. The theory can be conceived as an extension of linear integer/real arithmetic with a weakly-axiomatized multiplication symbol, which retains many of the desirable algorithmic properties of linear arithmetic. In particular, we show that the conjunctive fragment of the theory can be effectively manipulated (analogously to the usual operations on convex polyhedra, the conjunctive fragment of linear arithmetic). As a result, we can solve the following consequence-finding problem: given a ground formula F, find the strongest conjunctive formula that is entailed by F. As an application of consequence-finding, we give a loop invariant generation algorithm that is monotone with respect to the theory and (in a sense) complete. Experiments show that the invariants generated from the consequences are effective for proving safety properties of programs that require non-linear reasoning.

==> pratenddefaultcategory.tex <==


\prAtEndRestateii*

\makeatletter\Hy@SaveLastskip\pratendChangeCurrentLabel\label{proofsection:prAtEndii}\Hy@RestoreLastskip\makeatother\begin{proof}[Proof]\phantomsection\label{proof:prAtEndii}Since $1 \in L$, $1 + I \in \Int ^{\ConeModel {C, L}}$ and $\ConeModel {C, L} \models \Int (1)$. The closure axioms hold because $L$ is closed under addition and taking additive inverses. \par For the cutting plane axiom, let $n, m \in \mathbb {Z}$, $n > 0$, and $p \in \mathbb {Z}[X]$ be such that $np + m \in C$ and $p \in L$. Since $C$ is closed under cutting planes with respect to $L$, $p + \floor {\frac {m}{n}} \in C$. So $\ConeModel {C, L} \models 0 \leq p + \floor {\frac {m}{n}}$.\end{proof}

\prAtEndRestateiii*

\makeatletter\Hy@SaveLastskip\pratendChangeCurrentLabel\label{proofsection:prAtEndiii}\Hy@RestoreLastskip\makeatother\begin{proof}[Proof]\phantomsection\label{proof:prAtEndiii}Sufficiency follows from Lemma~\ref {lem:thz-model-construction}. For necessity, assume $F$ to be satisfiable, and consider some $\ThZ $-model $M$ that satisfies $F$. Following the proof of Theorem~\ref {thm:min-model-for-conjunction}, $\CnM {M} = \set {p \in \mathbb {Q}[X]: M \models 0 \leq p}$ is a regular cone that contains $P$. \par Consider $np + m \in \CnM {M}$, where $n, m \in \mathbb {Z}$, $n > 0$, and $p \in \product {\mathbb {Z}}{B}$. Since $M \models \Int (s)$ for all $s \in S$ and $M \models \Int (1)$, by the $\Int $ closure axioms, $M \models \Int (p)$. Since $M$ satisfies the cutting plane axiom, $M \models p + \floor {\frac {m}{n}} \geq 0$. Hence, $p + \floor {\frac {m}{n}} \in \CnM {M}$. \par Thus, $C \subseteq \CnM {M}$. As per the proof of Theorem~\ref {thm:min-model-for-conjunction}, $C$ is consistent, and $\ConeModel {C, \units {C} + \product {\mathbb {Z}}{B}}$ satisfies $0 \leq p$, $\lnot (0 \leq q)$, and $\lnot (0 = r)$ for all $p \in P$, $q \in Q$ and $r \in R$. It satisfies all $\Int (s)$ since each $s \in B$. If $\ConeModel {C, \units {C} + \product {\mathbb {Z}}{B}} \models \Int (t)$ for some $t \in T$, then $t \in \units {C} + \product {\mathbb {Z}}{B}$, i.e., $t = z + b$ for some $z \in \units {C}$ and $b \in \product {\mathbb {Z}}{B}$. Since $C \subseteq \CnM {M}$, $M \models z = 0$. Since $M \models \Int (0)$ and $M \models \Int (b)$, $M \models \Int (t)$, contradicting $M \models F$. So $\ConeModel {C, \units {C} + \product {\mathbb {Z}}{B}} \models \lnot \Int (t_k)$. Thus, it satisfies $F$.\end{proof}

\prAtEndRestateiv*

\makeatletter\Hy@SaveLastskip\pratendChangeCurrentLabel\label{proofsection:prAtEndiv}\Hy@RestoreLastskip\makeatother\begin{proof}[Proof]\phantomsection\label{proof:prAtEndiv}Let $T = \set {y - f(y) : y \in Y}$. Expanding the definition of \textit {inverse-hom} and using Theorem~\ref {thm:projection}, $\algconeX {\textit {inverse-hom}(Z,P,f,Y)}{Y} = \algconeX {T \cup Z, P}{X, Y} \cap \mathbb {Q}[Y]$. \par ($\subseteq $) If $s \in \algconeX {T \cup Z, P}{X, Y} \cap \mathbb {Q}[Y]$, then $s - p \in \product {\mathbb {Q}[X, Y]}{T \cup Z}$ for some $p \in \product {\Qplus }{P}$. \par Extend the ring homomorphism $f: \mathbb {Q}[Y] \to \mathbb {Q}[X]$ to a homomorphism $\hat {f}: \mathbb {Q}[X, Y] \to \mathbb {Q}[X]$ such that $\hat {f}(x) = x$ for each variable $x \in X$ and $\hat {f}(y) = f(y)$ for each variable $y \in Y$, so that $\hat {f} |_{\, \mathbb {Q}[Y]} = f$. By Lemma~\ref {lem:eval-ring-hom}, and noting that $T = \set {y - f(y) : y \in Y} = \set {y - \hat {f}(y) : y \in Y}$, $\hat {f}(s-p) - (s - p) \in \product {\mathbb {Q}[X]}{T \cup Z}$. \par Then $\hat {f}(s - p) = (\hat {f}(s-p) - (s - p)) + (s - p) \in \product {\mathbb {Q}[X]}{T \cup Z}$. Since $Z \subseteq \mathbb {Q}[X]$ is a Gr\"{o}bner basis and $X \cap Y = \emptyset $, $T \cup Z$ is a Gr\"{o}bner basis for $\product {\mathbb {Q}[X]}{T \cup Z}$ with respect to an elimination order $\preceq _X$. Since $\hat {f}(s - p) \in \mathbb {Q}[X]$, by the ordering property of Gr\"{o}bner bases, $\hat {f}(s - p) \in \product {\mathbb {Q}[X]}{Z}$. Then $f(s) = \hat {f}(s) = \hat {f}(s - p) + \hat {f}(p) = \hat {f}(s - p) + p \in \algconeX {Z, P}{X}$. \par \par ($\supseteq $) Let $p \in \mathbb {Q}[Y]$ be such that $f(p) \in \algconeX {Z, P}{X}$. By considering the extended ring homomorphism $\hat {f}$ above, we have by Lemma~\ref {lem:eval-ring-hom} that $p - f(p) \in \product {\mathbb {Q}[X, Y]}{T}$. Since $f(p) \in \algconeX {Z, P}{X}$, $p = (p - f(p)) + f(p) \in \product {\mathbb {Q}[X,Y]}{T} + \algconeX {Z,P}{X} \subseteq \algconeX {Z \cup T,P}{X,Y}$.\end{proof}

\prAtEndRestatev*

\makeatletter\Hy@SaveLastskip\pratendChangeCurrentLabel\label{proofsection:prAtEndv}\Hy@RestoreLastskip\makeatother\begin{proof}[Proof]\phantomsection\label{proof:prAtEndv}Let $T = \set {y - \hat {g}(y): y \in Y}$. Let $C = \algconeX {Z, P}{X}$. For $\subseteq $, $\algconeX {T \cup Z, P}{X, Y} \cap \linpoly {Y} \subseteq \algconeX {T \cup Z, P}{X, Y} \cap \mathbb {Q}[Y] = \hat {g}^{-1}(C)$, so $g(\algconeX {T \cup Z, P}{X, Y} \cap \linpoly {Y}) \subseteq C$. For $\supseteq $, note that $g^{-1}(C) \subseteq \hat {g}^{-1}(C) \subseteq \algconeX {T \cup Z, P}{X, Y}$, and $g^{-1}(\algconeX {Z, P}{X}) \subseteq \linpoly {Y}$ by definition.\end{proof}

\prAtEndRestatevi*

\makeatletter\Hy@SaveLastskip\pratendChangeCurrentLabel\label{proofsection:prAtEndvi}\Hy@RestoreLastskip\makeatother\begin{proof}[Proof]\phantomsection\label{proof:prAtEndvi}By Corollary~\ref {cor:inverse-linear-groebner}, the definition of \textit {intersect-subspace}, and Theorem~\ref {thm:intersection}, \[ \product {\Qplus }{\textit {intersect-subspace}(\textit {inverse-hom}(Z, P, \hat {f}, Y), Y)} = f^{-1}(\algconeX {Z, P}{X}))). \] \par Let $P_1 = \textit {intersect-subspace}(\textit {inverse-hom}(Z, P, \hat {f}, Y), Y)$. The $\polyhedralcut $ procedure computes cutting plane closure, so $\product {\Qplus }{\polyhedralcut (P_1)} = \cp _{\, \product {\mathbb {Z}}{Y}}(\product {\Qplus }{P_1})$. \par Let $P_2 = \polyhedralcut (P_1)$. Then \[ \begin {array}{llr} \product {\Qplus }{\textit {substitute}(\hat {f}, P_2)} &= \product {\Qplus }{\set {\hat {f}(p) : p \in P_2}} & \\ &= \product {\Qplus }{\set {f(p) : p \in P_2}} & \text { since $Z_3, P_3 \subseteq \linpoly {Y}$}\\ &= f(\product {\Qplus }{P_2}) & \text { by linearity of $f$}. \end {array} \] Chaining these parts yields the claim.\end{proof}

\prAtEndRestatevii*

\makeatletter\Hy@SaveLastskip\pratendChangeCurrentLabel\label{proofsection:prAtEndvii}\Hy@RestoreLastskip\makeatother\begin{proof}[Proof]\phantomsection\label{proof:prAtEndvii}Let $B_0^{(i)}$ be $B'$ at the start of the $i$-th iteration. Let $Z_0^{(i)}$ and $C^{(i)}$ be $Z_0$ and $\regcone (Z_0, P_0)$ in the $i$-th iteration respectively. By Theorem~\ref {thm:saturation}, Lemma~\ref {lem:cp-ineq-closure} and Lemma~\ref {lem:cut-correct}, $C^{(i+1)} = R(\cp _{\, \product {\mathbb {Z}}{B_0^{(i)}}}(C^{(i)}))$, where $R(C)$ is the least regular cone containing $C$. We first claim that for all $0 \leq i \leq j$, \begin {align*} \cp _{\, \product {\mathbb {Z}}{B_0^{(i)}}}(C^{(j)}) = \cp _{\, \product {\mathbb {Z}}{B}}(C^{(j)}). \end {align*} Then in particular, $C^{(i+1)} = R(\cp _{\, \product {\mathbb {Z}}{B}}(C^{(i)}))$. By Lemma~\ref {lem:saturate-cp-closure}, the algorithm terminates with $\regcone (Z', P')$ as the least regular cone $C$ that contains $\regcone (Z, P)$ and is closed under cutting planes with respect to $\product {\mathbb {Z}}{B}$. By Lemma~\ref {lem:cp-ineq-invariance}, it is closed under cutting planes with respect to $\units {\regcone (Z', P')} + \product {\mathbb {Z}}{B}$. If $C'$ is any regular cone containing $\regcone (Z, P)$ and is closed under cutting planes with respect to $\units {C'} + \product {\mathbb {Z}}{B}$, it is in particular closed under cutting planes with respect to $\product {\mathbb {Z}}{B}$, so $\regcone (Z', P') \subseteq C'$. This proves the theorem. \par We prove the claim by induction on $i$. The base case follows by noting that $\product {\mathbb {Z}}{B} = \product {\mathbb {Z}}{B_0^{(0)}}$. Now assume the induction hypothesis, i.e., for all $j$ such that $0 \leq i \leq j$, $\cp _{\, \product {\mathbb {Z}}{B_0^{(i)}}}(C^{(j)}) = \cp _{\, \product {\mathbb {Z}}{B}}(C^{(j)})$. We wish to show that if $i + 1 \leq j$, $\cp _{\, \product {\mathbb {Z}}{B_0^{(i+1)}}}(C^{(j)}) = \cp _{\, \product {\mathbb {Z}}{B}}(C^{(j)})$. Each $b^{(i+1)} \in B_0^{(i+1)}$ is obtained by reducing $B_0^{(i)}$ using $Z_0^{(i+1)}$ and computing a basis, so $b^{(i+1)} = \sum _k a_k (b_k^{(i)} - z_k^{(i+1)})$, where each $a_k \in \mathbb {Z}$, $b_k^{(i)} \in B_0^{(i)}$, and $z_{k}^{(i+1)} \in \qideal {Z_0^{(i+1)}}$. Since $i + 1 \leq j$ and $\units {C^{(i+1)}} \subseteq \units {C^{(j)}}$, $\product {\mathbb {Z}}{B_0^{(i+1)}} \subseteq \units {C^{(i+1)}} + \product {\mathbb {Z}}{B_0^{(i)}} \subseteq \units {C^{(j)}} + \product {\mathbb {Z}}{B_0^{(i)}}$. Symmetrically, each $b^{(i)} = z^{(i+1)} + \sum _k a_k b_k^{(i+1)}$, where each $a_k \in \mathbb {Z}$, $b_k^{(i+1)} \in B_0^{(i+1)}$, and $z^{(i+1)} \in Z_0^{(i+1)}$. Hence, $\product {\mathbb {Z}}{B_0^{(i)}} \subseteq \units {C^{(j)}} + \product {\mathbb {Z}}{B_0^{(i+1)}}$. By Lemma~\ref {lem:cp-ineq-invariance}, $\cp _{\, \product {\mathbb {Z}}{B_0^{(i+1)}}}(C^{(j)}) = \cp _{\, \product {\mathbb {Z}}{B_0^{(i)}}}(C^{(j)})$. By the induction hypothesis, the claim follows.\end{proof}

\prAtEndRestateviii*

\makeatletter\Hy@SaveLastskip\pratendChangeCurrentLabel\label{proofsection:prAtEndviii}\Hy@RestoreLastskip\makeatother\begin{proof}[Proof]\phantomsection\label{proof:prAtEndviii}Without loss of generality we may assume that $\tuple {Z, P}$ is reduced w.r.t. $\preceq _K$. The $\subseteq $ inclusion is obvious, since by construction $V$ is a subset of $\units {\regcone (Z,P)}$ and $\mathbb {Q}[K]$, and $R$ is a subset of $\regcone (Z,P)$ and $(\mathbb {Q}[K] + \product {\mathbb {Q}}{D})$. \par For the $\supseteq $ direction, suppose $q \in \regcone (Z,P) \cap (\mathbb {Q}[K] + \product {\mathbb {Q}}{D})$. Thus $q \in (\mathbb {Q}[K] + \product {\mathbb {Q}}{D})$ can be written as $q = z + p$ for $z \in \product {\mathbb {Q}[D,K]}{Z}$, $p \in \cone {P}$. According to \autoref {lem:decomp-to-smaller-monos}, $\leadmon (z) \preceq _K \leadmon (q)$ and $\leadmon (p) \preceq _K \leadmon (q)$. Thus $p \in \cone {P} \cap (\mathbb {Q}[K] + \product {\mathbb {Q}}{D}) \subseteq \cone {R}$, since $\cone {R} = \cone {P} \cap (\mathbb {Q}[K] + \product {\mathbb {Q}}{D})$ by properties of cone projection in Section~\ref {sec:subsub-proj-alg-cones}. We thus only need to show that $z \in \cone {R} + \product {\mathbb {Q}[K]}{V}$. \par Suppose $z = q_1z_1 + \dots + q_nz_n$ for $q_1, \dots , q_n \in \mathbb {Q}[D, K]$ and $z_1, \dots , z_n \in Z$. Then $\leadmon (q_iz_i) \preceq _K \leadmon (z)$ for all $i$. Next we proceed based on what $\leadmon (z_i)$ looks like for each $i$. \par If $\leadmon (z_i) \in \mathbb {Q}[K]$. In this case $q_i$ must not involve any variable $D$, since otherwise $\leadmon (q_i z_i)$ will be ranked higher than anything in $(\mathbb {Q}[K] + \product {\mathbb {Q}}{D})$ including $\leadmon (z)$ w.r.t. the monomial ordering $\preceq _K$. In other words $q_i \in \mathbb {Q}[K]$. This $z_i$ is added to $V$, thus $q_i z_i \in \product {\mathbb {Q}[K]}{V}$. \par If $\leadmon (z_i)$ contains any variable in $D$, then $q_i \in \mathbb {Q}$ for the same reason as above. In this case $q_i z_i \in \cone {R}$ since $z_i$ and $-z_i$ are added to $R$.\end{proof}

